Structure-preserving neural networks for the regularized entropy-based closure of the Boltzmann moment system

The main challenge of large-scale numerical simulation of radiation transport is the high memory and computation time requirements of discretization methods for kinetic equations. In this work, we derive and investigate a neural network-based approximation to the entropy closure method to accurately compute the solution of the multi-dimensional moment system with a low memory footprint and competitive computational time. We extend methods developed for the standard entropy-based closure to the context of regularized entropy-based closures. The main idea is to interpret structure-preserving neural network approximations of the regularized entropy closure as a two-stage approximation to the original entropy closure. We conduct a numerical analysis of this approximation and investigate optimal parameter choices. Our numerical experiments demonstrate that the method has a much lower memory footprint than traditional methods with competitive computation times and simulation accuracy.

==> assets/algorithms/alg_network_inference.tex <==
\DontPrintSemicolon
\caption{Rotation invariant network inference within a kinetic solver}
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwComment{Comment}{$\triangleright$\ }{}



\Input{$\fu_i$: Full moments $\fu\in\mathbb{R}^n$ of the computational grid grid $\widetilde{\mathbf{X}}$\newline}
\KwResult{${f^p_{\fu_i}}$: Reconstructed, regularized kinetic densities of the grid $\widetilde{\mathbf{X}}$\newline }


\For {each $\ofu_i \in \widetilde{\mathbf{X}}$}{


%$\hat{h}_i^p\gets \hat{h}^p(\overline{\fu}_{\#,i}),$\tcc*[r]{Entropy approximation}
$\fw\gets \ofu_{\#,i}$ \\
$\fz^\pm\gets  Z^\pm(\fw)$ \tcc*[r]{Rotation}
$\bm\beta_{\overline{\fu}_{\#,i}}^p \gets  0.5\left(\nabla_\fw Z^+(\fw)\nabla_\fz \check{h}^p(\fz^+)+\nabla_\fw Z^-(\fw)\nabla_\fz \check{h}^p(\fz^-)\right)$\tcc*[r]{Lagrange multiplier approximation}
%$\nabla_\fw\fz_{\ofus_i} \gets \nabla_\fw \fz(\ofus_i)$\tcc*[r]{Compute rotation gradient}
$ \mathbf{g}_{{\fu}_i}^p\gets \left[\hat{h}^p(\overline{\fu}_{\#,i}) - (\ofus_{,i})\cdot \bm\beta_{\overline{\fu}_{\#,i}}^p +\log u_{0,i} + 1,\,(\bm\beta_{\overline{\fu}_{\#,i}}^{p})^\top \right]^\top$\tcc*[r]{Gradient reconstruction}

$f^p_{{\fu}_i}\gets\exp\left(\mathbf{g}_{{\fu}_i}^p\cdot\mathbf m\right)$\tcc*[r]{Kinetic density reconstruction}

%$f^p_{{\fu},i}\gets u_{0,i}f^p_{\overline{\fu},i}$.\tcc*[r]{Re-scale kinetic density}
}






==> assets/algorithms/alg_network_inference_reflection.tex <==
\DontPrintSemicolon
\caption{Rotation and reflection invariant network inference within a kinetic solver for the M$_1$ closure}
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwComment{Comment}{$\triangleright$\ }{}



\Input{$\fu_i$: M$_1$ moments of the grid $\widetilde{\mathbf{X}}$\newline}
\KwResult{${f^p_{\fu,i}}$: Reconstructed, regularized kinetic densities of the grid $\widetilde{\mathbf{X}}$\newline }

\For {each $\fu_i \in \widetilde{\mathbf{X}}$}{

$\overline{\fu}_i^+\gets M_{R_{\mathbf{V}_{1,+}}}\overline{\fu}_i$ \tcc*[r]{Rotate moment onto $\mathbf{V}_{1,+}$}

$\overline{\fu}_i^-\gets M_{R_\pm} M_{R_{\mathbf{V}_{1,+}}}\overline{\fu}_i$ \tcc*[r]{Rotate moment onto $\mathbf{V}_{1,-}$}

%$\hat{h}_i^{p,+},\,\hat{h}_i^{p,-}\gets\hat{h}^{p}\left((\overline{\fu}_i^+)_\#\right),\, \hat{h}^{p}\left((\overline{\fu}_i^-)_\#\right)$\tcc*[r]{Entropy approximations}

$\bm\beta_{\overline{\fu}_{\#,i}^+}^{p},\,\bm\beta_{\overline{\fu}_{\#,i}^-}^{p}\gets\nabla_{\overline{\fu}^+_{\#}}\hat{h}^{p}\left((\overline{\fu}_i^+)_\#\right),\,\nabla_{\overline{\fu}^-_{\#}}\hat{h}^{p}\left((\overline{\fu}_i^-)_\#\right)$\tcc*[r]{Lagrange multiplier approximations}


$\bm\beta_{\overline{\fu}_{\#,i}}^{p,\text{sym}}\gets \frac{1}{2}\left(\bm\beta_{\overline{\fu}_{\#,i}^+}^{p}+(M_{R_\pm}^\top)_\#\bm\beta_{\overline{\fu}_{\#,i}^-}^{p}\right)$\tcc*[r]{Average}

$\bm\beta_{\overline{\fu}_{\#,1}}^{p,\text{sym}}\gets 0$\tcc*[r]{Reflection invariance}


$\bm\beta_{\overline{\fu}_{\#,i}}^{p}\gets \left(M_{R_{\mathbf{V}_{1,+}}}\right)_\#^\top\bm\beta_{\overline{\fu}_{\#,i}}^{p,\text{sym}} $\tcc*[r]{Reverse rotation}


$\hat{h}^p_i\gets \frac{1}{2}\left( \hat{h}^{p}\left((\overline{\fu}_i^+)_\#\right) +\hat{h}^{p}\left((\overline{\fu}_i^-)_\#\right) \right)$\tcc*[r]{Reconstruct averaged entropy}


$ \mathbf{g}_{{\fu}_i}^p\gets \left[ \hat{h}^p_i- (\overline{\fu}_\#)^\top \nabla_{{\fu}_\#}\hat{h}^p(\overline{\fu}_\#) +\log u_0 + 1 ,(\bm\beta_{\overline{\fu}_{\#,i}}^{p})^\top \right]^\top$\tcc*[r]{Reconstruct full entropy gradient}

$f^p_{\overline{\fu},i}\gets\exp\left(\mathbf{g}_{{\fu}_i}^p\cdot\mathbf m\right)$\tcc*[r]{Reconstruct kinetic density}

}




==> assets/img/tikz/notation.tex <==

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Rectangle [id:dp4163502009222797] 
\draw   (165,109) -- (344,109) -- (344,290) -- (165,290) -- cycle ;
%Shape: Rectangle [id:dp23956609812377483] 
\draw  [fill={rgb, 255:red, 196; green, 196; blue, 196 }  ,fill opacity=1 ] (165,109) -- (184,109) -- (184,130) -- (165,130) -- cycle ;
%Shape: Rectangle [id:dp008065915774243537] 
\draw  [fill={rgb, 255:red, 196; green, 196; blue, 196 }  ,fill opacity=1 ] (184,130) -- (244,130) -- (244,189) -- (184,189) -- cycle ;
%Shape: Rectangle [id:dp21357303951049844] 
\draw  [fill={rgb, 255:red, 196; green, 196; blue, 196 }  ,fill opacity=1 ] (244,189) -- (344,189) -- (344,290) -- (244,290) -- cycle ;
%Straight Lines [id:da33589358294944205] 
\draw    (164,99) -- (344,99) ;
\draw [shift={(344,99)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
\draw [shift={(164,99)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
%Shape: Rectangle [id:dp3742934554770203] 
\draw   (365,109) -- (384,109) -- (384,289) -- (365,289) -- cycle ;
%Straight Lines [id:da6838359078522513] 
\draw    (395,109) -- (395,289) ;
\draw [shift={(395,289)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
\draw [shift={(395,109)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
%Shape: Rectangle [id:dp7786624861855411] 
\draw   (365,109) -- (384,109) -- (384,130) -- (365,130) -- cycle ;
%Shape: Rectangle [id:dp588477696396051] 
\draw   (365,190) -- (384,190) -- (384,289) -- (365,289) -- cycle ;
%Straight Lines [id:da7562531166367892] 
\draw    (185,88) -- (344,88) ;
\draw [shift={(344,88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
\draw [shift={(185,88)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
%Straight Lines [id:da8602025636128408] 
\draw    (246,78) -- (344,78) ;
\draw [shift={(344,78)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
\draw [shift={(246,78)}, rotate = 180] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
%Straight Lines [id:da663950597656624] 
\draw    (405,129) -- (405,289) ;
\draw [shift={(405,289)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
\draw [shift={(405,129)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
%Straight Lines [id:da35872542672895413] 
\draw    (415,189) -- (415,289) ;
\draw [shift={(415,289)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
\draw [shift={(415,189)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (0,5.59) -- (0,-5.59)   ;
%Straight Lines [id:da7494866733042838] 
\draw    (62,90) -- (155.01,99.79) ;
\draw [shift={(157,100)}, rotate = 186.01] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da9571296336313384] 
\draw    (182,60) -- (218.35,84.87) ;
\draw [shift={(220,86)}, rotate = 214.38] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da01769455790967367] 
\draw    (279,55) -- (279,73) ;
\draw [shift={(279,75)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (532,146) node [anchor=north west][inner sep=0.75pt]   [align=left] {$ $};
% Text Node
\draw (267,29) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle M_{R}^{\#\#} \in \mathbb{R}^{( n-3) \times ( n-3)}$};
% Text Node
\draw (417,192) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \overline{\mathbf{u}}_{\#\#} \in \mathbb{R}^{n-3}$};
% Text Node
\draw (407,132) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \overline{\mathbf{u}}_{\#} \in \mathbb{R}^{n}$};
% Text Node
\draw (391,86) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \overline{\mathbf{u}} \in \mathbb{R}^{n+1}$};
% Text Node
\draw (165,34) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle M_{R}^{\#} \in \mathbb{R}^{n\times n}$};
% Text Node
\draw (26,65) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle M_{R} \in \mathbb{R}^{( n+1) \times ( n+1)}$};
% Text Node
\draw (367,112) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle \overline{\mathbf{u}}_{0}$};
% Text Node
\draw (365,152) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle \overline{\mathbf{u}}_{1}$};
% Text Node
\draw (365,233) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle \overline{\mathbf{u}}_{2}$};


\end{tikzpicture}
